Applicability Evaluation of Selected xAI Methods for Machine Learning Algorithms for Signal Parameters Extraction

Machine learning methods find growing application in the reconstruction and analysis of data in high energy physics experiments. A modified convolutional autoencoder model was employed to identify and reconstruct the pulses from scintillating crystals. The model was further investigated using four xAI methods for deeper understanding of the underlying reconstruction mechanism. The results are discussed in detail, underlining the importance of xAI for knowledge gain and further improvement of the algorithms.

==> IG.tex <==
\subsection{Integrated Gradients}

The Integrated Gradients xAI method was developed as a tool to assess the dependence of neural network predictions to the input data features. It uses a defined baseline, which in the one-dimensional data case is a vector of same length as the input data, composed entirely of zeroes. The gradient between each point and the baseline is calculated with all gradients then being integrated as shown in Eq.\ref{eq:intgrad}.

\begin{equation}
    \text{IntegratedGradients}_{i}(x) ::= (x_{i} - x'_{i}) \times \int_{\alpha=0}^{1} \frac{\partial F(x' + \alpha \times (x - x'))}{\partial x_{i}} \, d\alpha~\cite{bib:intgrad}
    \label{eq:intgrad}
\end{equation}

In practice, the input is scaled with a certain step and the integral is calculated as the sum of the gradients for all scaled instances, as shown in Eq.\ref{eq:intgradapprox}.

\begin{equation}
    \text{IntegratedGrads}^{\text{approx}}_{i}(x) ::= (x_{i} - x'_{i}) \times \sum_{k=1}^{m} \frac{\partial F\left(x' + \frac{k}{m} \times (x - x')\right)}{\partial x_{i}} \times \frac{1}{m}~\cite{bib:intgrad}
    \label{eq:intgradapprox}
\end{equation}

The Integrated Gradients method finds application in a wide range of machine learning tasks, mainly in two-dimensional cases like image processing and classification. 
The input was divided in 1000 steps for the integral approximation, i.e. 
m=1000, $x_i' = 0$, and eq. \ref{eq:intgradapprox} reads
\begin{equation}
    \text{IntegratedGrads}^{\text{approx}}_{i}(x) ::= \frac{1}{m} \times x_{i} \times \sum_{k=1}^{m} \frac{\partial F\left(\frac{k}{m} \times x \right)}{\partial x_{i}} 
    \label{eq:intgradapprox-reduced}
\end{equation}
For all three models, the shape of the resulting curve replicates the waveform. 
However, for M(18, ReLu) the result shows the highest gradient values, 
while for M(18, lin) they are smaller and even negative for M(14, lin), which has a smaller kernel size for the filter in the last layer, compared to M(18, lin) and M(18, ReLu).
The results of applying the Integrated Gradients method for the modified autoencoders used for scintillating crystals data reconstruction are shown on Figure~\ref{fig:intgrad}. 
As it can be seen, the Integrated Gradients repeat the input waveform, 
with a constant scale factor, which indicates that 
\begin{equation}
    G_i = \sum_{k=1}^{m} \frac{\partial F\left(\frac{k}{m} \times x \right)}{\partial x_{i}}  =  const
\end{equation}
and does not depend on the 
position in the waveform. 
%WHY

\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{Figures/IntGrads_new.pdf}
\caption{Results from applying the Integrated Gradients method to the predictions from the three modified autoencoder models. M(18, ReLu), which uses ReLu activation shows the highest gradient values, while M(14, lin), which has a smaller kernel size for the filter in its last layer than the other two models, has negative values. 
\label{fig:intgrad}}
\end{figure}

